LangSAMP: Language-Script Aware Multilingual Pretraining

Recent multilingual pretrained language models (mPLMs) often avoid using language embeddings -- learnable vectors assigned to individual languages. However, this places a significant burden on token representations to encode all language-specific information, which may hinder language neutrality. To address this limitation, we propose Language-Script Aware Multilingual Pretraining (LangSAMP), a method that incorporates both language and script embeddings to enhance representation learning. Specifically, we integrate these embeddings into the output of the Transformer blocks before passing the final representations to the language modeling head for prediction. We apply LangSAMP to the continual pretraining of XLM-R on a highly multilingual corpus covering more than 500 languages. The resulting model consistently outperforms the baseline in zero-shot crosslingual transfer across diverse downstream tasks. Extensive analysis reveals that language and script embeddings capture language- and script-specific nuances, which benefits more language-neutral representations, proven by improved pairwise cosine similarity. In our case study, we also show that language and script embeddings can be used to select better source languages for crosslingual transfer. We make our code and models publicly available at https://github.com/cisnlp/LangSAMP.

==> bible_donor.tex <==
\begin{table*}
\centering
\setlength{\tabcolsep}{0.7mm}{}
\resizebox{\textwidth}{!}{
    \begin{tabular}{lrr|lrr|lrr|lrr}
    \toprule
    Language & English & Closest donor &     Language & English & Closest donor &     Language & English & Closest donor &     Language & English & Closest donor \\
    \midrule
ace\_Latn & 53.1 & \textbf{59.1} & ach\_Latn & \textbf{44.4} & 12.0 & acr\_Latn & 23.6 & \textbf{9.8} & afr\_Latn & \textbf{98.7} & 73.1 \\
ahk\_Latn & 3.8 & \textbf{6.9} & aka\_Latn & \textbf{64.7} & 53.1 & aln\_Latn & \textbf{96.7} & 90.7 & als\_Latn & \textbf{62.9} & 62.9 \\
alz\_Latn & 41.3 & \textbf{46.7} & amh\_Ethi & \textbf{72.0} & 72.0 & amh\_Latn & \textbf{4.9} & 4.9 & aoj\_Latn & 23.8 & \textbf{24.2} \\
arn\_Latn & \textbf{27.8} & 24.9 & ary\_Arab & 12.4 & \textbf{50.2} & arz\_Arab & 33.6 & \textbf{99.8} & asm\_Beng & 73.8 & \textbf{85.1} \\
azb\_Arab & \textbf{81.8} & 23.3 & azb\_Latn & \textbf{95.6} & 17.8 & aze\_Cyrl & \textbf{24.7} & 21.8 & aze\_Latn & \textbf{95.8} & 93.1 \\
bam\_Latn & \textbf{56.0} & 44.4 & ban\_Latn & \textbf{34.0} & 30.9 & bar\_Latn & \textbf{45.6} & 35.1 & bba\_Latn & \textbf{43.1} & 14.9 \\
bci\_Latn & 11.6 & \textbf{11.8} & bcl\_Latn & \textbf{82.9} & 78.9 & bel\_Cyrl & \textbf{94.0} & 93.1 & bem\_Latn & \textbf{77.8} & 18.9 \\
bhw\_Latn & \textbf{46.7} & 14.4 & bim\_Latn & 47.3 & \textbf{50.4} & bis\_Latn & \textbf{36.4} & 19.1 & bod\_Tibt & \textbf{50.9} & 25.8 \\
bre\_Latn & \textbf{22.9} & 21.3 & bts\_Latn & \textbf{70.4} & 69.6 & btx\_Latn & 59.3 & \textbf{67.8} & bul\_Cyrl & \textbf{98.9} & 96.7 \\
bzj\_Latn & \textbf{62.4} & 12.7 & cab\_Latn & 11.1 & \textbf{12.4} & cac\_Latn & 15.3 & \textbf{8.2} & cak\_Latn & 17.3 & \textbf{19.8} \\
cat\_Latn & \textbf{95.6} & 93.6 & cbk\_Latn & \textbf{57.3} & 54.4 & cce\_Latn & \textbf{49.6} & 17.8 & ceb\_Latn & \textbf{89.8} & 80.4 \\
cfm\_Latn & \textbf{61.1} & 14.4 & che\_Cyrl & 14.2 & \textbf{14.9} & chk\_Latn & \textbf{50.2} & 20.7 & chv\_Cyrl & 66.4 & \textbf{70.2} \\
cmn\_Hani & \textbf{92.9} & 44.7 & cnh\_Latn & \textbf{53.8} & 28.0 & crh\_Cyrl & \textbf{85.8} & 80.4 & crs\_Latn & \textbf{86.4} & 59.3 \\
ctd\_Latn & 62.0 & \textbf{64.4} & ctu\_Latn & \textbf{13.6} & 13.3 & cuk\_Latn & \textbf{19.8} & 17.3 & cym\_Latn & \textbf{47.3} & 41.6 \\
deu\_Latn & \textbf{96.7} & 96.7 & djk\_Latn & \textbf{33.1} & 16.4 & dln\_Latn & \textbf{68.2} & 68.2 & dtp\_Latn & 24.2 & \textbf{9.8} \\
dzo\_Tibt & \textbf{37.8} & 20.9 & efi\_Latn & \textbf{88.2} & 56.4 & ell\_Grek & \textbf{76.9} & 52.2 & eng\_Latn & \textbf{100.0} & 100.0 \\
epo\_Latn & \textbf{86.2} & 86.2 & est\_Latn & \textbf{94.4} & 80.0 & eus\_Latn & 16.9 & \textbf{18.9} & ewe\_Latn & \textbf{46.2} & 31.6 \\
fas\_Arab & \textbf{98.4} & 90.9 & fij\_Latn & \textbf{72.2} & 40.7 & fil\_Latn & \textbf{86.7} & 82.9 & fin\_Latn & \textbf{96.2} & 80.7 \\
fra\_Latn & \textbf{97.1} & 97.1 & fry\_Latn & \textbf{62.7} & 45.3 & gaa\_Latn & 70.0 & \textbf{75.3} & gil\_Latn & 38.2 & \textbf{44.9} \\
gkn\_Latn & \textbf{25.8} & 19.6 & gkp\_Latn & \textbf{25.3} & 20.2 & gla\_Latn & \textbf{47.1} & 47.1 & gle\_Latn & \textbf{58.2} & 51.1 \\
gom\_Latn & \textbf{36.0} & 34.7 & gor\_Latn & \textbf{23.8} & 23.3 & grc\_Grek & \textbf{69.6} & 69.6 & guc\_Latn & 10.2 & \textbf{8.4} \\
guj\_Gujr & \textbf{84.9} & 84.7 & gur\_Latn & \textbf{27.8} & 12.9 & guw\_Latn & \textbf{71.3} & 27.6 & gya\_Latn & \textbf{42.4} & 25.8 \\
hat\_Latn & 87.1 & \textbf{88.7} & hau\_Latn & \textbf{70.2} & 58.0 & haw\_Latn & \textbf{38.2} & 32.9 & heb\_Hebr & \textbf{11.8} & 10.9 \\
hil\_Latn & \textbf{93.3} & 73.8 & hin\_Deva & \textbf{94.0} & 94.0 & hin\_Latn & 59.3 & \textbf{84.0} & hmo\_Latn & \textbf{78.9} & 18.7 \\
hnj\_Latn & \textbf{84.4} & 80.7 & hra\_Latn & \textbf{58.7} & 48.4 & hrv\_Latn & \textbf{97.8} & 95.1 & hui\_Latn & 35.1 & \textbf{38.9} \\
hus\_Latn & 17.8 & \textbf{18.2} & hye\_Armn & \textbf{97.8} & 93.3 & hye\_Latn & \textbf{8.9} & 11.1 & iba\_Latn & \textbf{84.4} & 81.6 \\
ifa\_Latn & \textbf{31.1} & 11.6 & ifb\_Latn & \textbf{33.3} & 10.9 & ikk\_Latn & \textbf{49.6} & 17.8 & ilo\_Latn & \textbf{67.3} & 64.7 \\
isl\_Latn & \textbf{62.2} & 56.9 & ita\_Latn & 96.7 & \textbf{98.2} & ium\_Laoo & \textbf{4.0} & 3.1 & ium\_Latn & \textbf{46.4} & 23.1 \\
ixl\_Latn & \textbf{8.9} & 8.0 & izz\_Latn & \textbf{24.4} & 22.2 & jam\_Latn & \textbf{52.4} & 50.9 & jav\_Latn & 57.3 & \textbf{57.8} \\
kaa\_Cyrl & \textbf{88.4} & 88.0 & kaa\_Latn & 53.1 & \textbf{54.7} & kab\_Latn & 12.7 & \textbf{9.1} & kac\_Latn & \textbf{32.4} & 27.6 \\
kan\_Knda & 66.7 & \textbf{68.4} & kan\_Latn & \textbf{8.9} & 7.8 & kat\_Geor & \textbf{93.8} & 76.7 & kaz\_Cyrl & 77.3 & \textbf{78.0} \\
kek\_Latn & \textbf{22.4} & 13.1 & khm\_Khmr & \textbf{68.9} & 68.9 & kia\_Latn & \textbf{51.3} & 14.7 & kik\_Latn & 75.6 & \textbf{87.6} \\
kir\_Cyrl & \textbf{93.3} & 91.6 & kjb\_Latn & \textbf{20.2} & 19.3 & kjh\_Cyrl & \textbf{59.6} & 15.3 & kmm\_Latn & \textbf{48.4} & 48.4 \\
kmr\_Latn & \textbf{84.7} & 72.2 & knv\_Latn & \textbf{17.6} & 14.2 & kor\_Hang & 95.6 & \textbf{98.0} & kor\_Latn & 5.6 & \textbf{7.1} \\
krc\_Cyrl & \textbf{83.3} & 81.8 & kri\_Latn & \textbf{52.0} & 24.9 & ksd\_Latn & 57.8 & \textbf{64.7} & kss\_Latn & 6.2 & \textbf{9.1} \\
kua\_Latn & 64.7 & \textbf{73.3} & lam\_Latn & \textbf{44.4} & 28.7 & lao\_Laoo & \textbf{71.8} & 63.3 & lat\_Latn & 84.0 & \textbf{90.4} \\
ldi\_Latn & \textbf{18.9} & 13.3 & leh\_Latn & \textbf{61.6} & 17.8 & lhu\_Latn & 4.2 & \textbf{6.9} & lin\_Latn & 88.2 & \textbf{96.7} \\
loz\_Latn & \textbf{52.4} & 14.7 & ltz\_Latn & \textbf{74.7} & 74.7 & lug\_Latn & \textbf{63.8} & 13.8 & luo\_Latn & 42.7 & \textbf{53.8} \\
lzh\_Hani & \textbf{75.8} & 75.8 & mad\_Latn & 44.2 & \textbf{47.8} & mah\_Latn & \textbf{39.1} & 16.0 & mai\_Deva & \textbf{62.0} & 17.8 \\
mal\_Mlym & 76.4 & \textbf{80.2} & mam\_Latn & 8.4 & \textbf{8.7} & mar\_Deva & 88.9 & \textbf{90.4} & mau\_Latn & 3.1 & \textbf{4.9} \\
mck\_Latn & \textbf{60.4} & 16.9 & mcn\_Latn & \textbf{47.3} & 34.2 & mco\_Latn & 5.6 & \textbf{8.9} & mdy\_Ethi & \textbf{39.8} & 31.3 \\
    \bottomrule
    \end{tabular}
}
    \caption{Top-10 accuracy of \frameworkname on \textbf{SR-B} using English and the closest donor language as source (Part I).}\label{tab:srb_donor_table1}
\end{table*}

\begin{table*}
\centering
\setlength{\tabcolsep}{0.7mm}{}
\resizebox{\textwidth}{!}{
    \begin{tabular}{lrr|lrr|lrr|lrr}
    \toprule
    Language & English & Closest donor &     Language & English & Closest donor &     Language & English & Closest donor &     Language & English & Closest donor \\
    \midrule
mfe\_Latn & \textbf{87.3} & 84.0 & mgh\_Latn & 18.7 & \textbf{25.3} & mgr\_Latn & 51.8 & \textbf{58.2} & mhr\_Cyrl & 55.8 & \textbf{56.7} \\
miq\_Latn & \textbf{44.2} & 44.2 & mkd\_Cyrl & \textbf{96.2} & 95.1 & mlg\_Latn & \textbf{76.0} & 73.1 & mlt\_Latn & \textbf{82.9} & 82.9 \\
mps\_Latn & \textbf{20.9} & 18.7 & mri\_Latn & 52.9 & \textbf{57.3} & mrw\_Latn & \textbf{51.6} & 46.9 & msa\_Latn & \textbf{91.8} & 90.4 \\
mxv\_Latn & 7.3 & \textbf{7.8} & mya\_Mymr & \textbf{61.3} & 36.4 & myv\_Cyrl & 38.0 & \textbf{39.8} & mzh\_Latn & \textbf{32.0} & 30.0 \\
naq\_Latn & \textbf{39.8} & 16.7 & nav\_Latn & \textbf{9.1} & 7.6 & nbl\_Latn & \textbf{72.7} & 72.7 & nch\_Latn & \textbf{19.1} & 14.4 \\
ndc\_Latn & \textbf{60.7} & 50.2 & nde\_Latn & \textbf{72.4} & 17.1 & ndo\_Latn & \textbf{53.8} & 15.1 & nds\_Latn & \textbf{56.9} & 47.6 \\
ngu\_Latn & \textbf{46.7} & 28.4 & nia\_Latn & \textbf{20.7} & 17.8 & nld\_Latn & \textbf{84.9} & 76.4 & nmf\_Latn & \textbf{50.7} & 49.8 \\
nno\_Latn & \textbf{95.6} & 95.6 & nob\_Latn & \textbf{97.3} & 88.2 & nor\_Latn & \textbf{97.8} & 89.8 & npi\_Deva & \textbf{80.4} & 79.6 \\
nso\_Latn & \textbf{80.4} & 80.4 & nya\_Latn & \textbf{76.9} & 14.0 & nyn\_Latn & 55.6 & \textbf{68.2} & nyy\_Latn & \textbf{19.6} & 17.6 \\
ori\_Orya & \textbf{61.6} & 61.6 & ory\_Orya & \textbf{77.8} & 74.0 & oss\_Cyrl & \textbf{64.2} & 46.9 & ote\_Latn & 11.1 & \textbf{11.3} \\
pam\_Latn & \textbf{50.7} & 43.3 & pan\_Guru & \textbf{66.2} & 66.2 & pap\_Latn & \textbf{91.6} & 89.3 & pau\_Latn & \textbf{23.6} & 23.3 \\
pdt\_Latn & \textbf{79.3} & 72.7 & pes\_Arab & \textbf{97.6} & 90.9 & pis\_Latn & \textbf{87.6} & 77.8 & pls\_Latn & 37.6 & \textbf{38.2} \\
poh\_Latn & \textbf{7.6} & 6.2 & pol\_Latn & \textbf{95.3} & 92.9 & pon\_Latn & \textbf{55.1} & 54.0 & por\_Latn & 98.4 & \textbf{99.1} \\
prs\_Arab & \textbf{95.1} & 89.6 & pxm\_Latn & \textbf{18.0} & 11.3 & qub\_Latn & \textbf{45.6} & 12.4 & quc\_Latn & \textbf{19.6} & 11.1 \\
quh\_Latn & \textbf{74.4} & 17.8 & quw\_Latn & \textbf{63.6} & 62.9 & quy\_Latn & 68.0 & \textbf{74.4} & quz\_Latn & \textbf{75.1} & 25.6 \\
rap\_Latn & \textbf{16.4} & 12.7 & rar\_Latn & 57.6 & \textbf{58.7} & rmy\_Latn & \textbf{42.0} & 38.4 & ron\_Latn & \textbf{97.1} & 92.7 \\
rug\_Latn & \textbf{46.4} & 15.1 & run\_Latn & 82.0 & \textbf{94.2} & rus\_Cyrl & \textbf{92.2} & 92.2 & sag\_Latn & \textbf{62.9} & 25.8 \\
san\_Arab & 2.9 & \textbf{3.1} & san\_Beng & \textbf{5.8} & 5.6 & san\_Deva & 31.6 & \textbf{34.2} & san\_Gujr & \textbf{6.4} & 5.1 \\
san\_Khmr & 2.7 & \textbf{2.9} & san\_Knda & 4.7 & \textbf{4.9} & san\_Latn & 10.7 & \textbf{11.6} & san\_Mlym & \textbf{6.4} & 5.3 \\
san\_Orya & 4.7 & \textbf{5.6} & san\_Sinh & \textbf{4.0} & 3.8 & san\_Taml & 2.0 & \textbf{3.1} & san\_Telu & \textbf{6.0} & 5.1 \\
san\_Tibt & 2.2 & \textbf{2.9} & sba\_Latn & \textbf{34.0} & 17.3 & seh\_Latn & \textbf{70.9} & 20.9 & sin\_Sinh & 63.1 & \textbf{78.4} \\
slv\_Latn & \textbf{95.3} & 89.6 & sme\_Latn & \textbf{53.3} & 16.4 & smo\_Latn & 27.1 & \textbf{31.3} & sna\_Latn & \textbf{70.2} & 44.2 \\
som\_Latn & \textbf{45.8} & 44.0 & sop\_Latn & \textbf{33.6} & 12.2 & sot\_Latn & \textbf{77.8} & 74.7 & spa\_Latn & \textbf{98.4} & 98.4 \\
srm\_Latn & 21.8 & \textbf{8.2} & srn\_Latn & \textbf{78.7} & 44.7 & srp\_Cyrl & \textbf{97.8} & 96.7 & srp\_Latn & \textbf{98.2} & 96.0 \\
sun\_Latn & 48.2 & \textbf{52.9} & suz\_Deva & \textbf{35.1} & 14.4 & swe\_Latn & \textbf{97.3} & 88.7 & swh\_Latn & \textbf{96.0} & 96.0 \\
tam\_Taml & \textbf{76.2} & 76.2 & tat\_Cyrl & \textbf{73.3} & 73.1 & tbz\_Latn & \textbf{37.3} & 17.8 & tca\_Latn & \textbf{20.9} & 10.9 \\
tel\_Telu & 71.6 & \textbf{78.9} & teo\_Latn & \textbf{36.9} & 35.6 & tgk\_Cyrl & \textbf{86.4} & 86.4 & tgl\_Latn & \textbf{93.6} & 69.8 \\
tih\_Latn & \textbf{48.7} & 14.4 & tir\_Ethi & \textbf{62.7} & 62.7 & tlh\_Latn & \textbf{94.2} & 94.2 & tob\_Latn & \textbf{15.3} & 13.3 \\
toi\_Latn & \textbf{57.6} & 43.6 & toj\_Latn & 10.4 & \textbf{10.7} & ton\_Latn & 20.9 & \textbf{24.0} & top\_Latn & 6.2 & \textbf{9.1} \\
tpm\_Latn & 27.3 & \textbf{8.7} & tsn\_Latn & \textbf{62.7} & 51.1 & tso\_Latn & \textbf{62.2} & 57.3 & tsz\_Latn & \textbf{27.6} & 14.4 \\
tui\_Latn & \textbf{34.9} & 34.9 & tuk\_Cyrl & \textbf{85.1} & 81.1 & tuk\_Latn & \textbf{83.1} & 82.2 & tum\_Latn & \textbf{71.8} & 21.1 \\
twi\_Latn & \textbf{64.4} & 47.1 & tyv\_Cyrl & 60.0 & \textbf{65.6} & tzh\_Latn & \textbf{21.1} & 19.1 & tzo\_Latn & \textbf{23.1} & 23.1 \\
uig\_Arab & 62.4 & \textbf{72.4} & uig\_Cyrl & 25.1 & \textbf{47.3} & uig\_Latn & 10.4 & \textbf{23.3} & ukr\_Cyrl & 94.4 & \textbf{94.9} \\
urd\_Deva & 58.7 & \textbf{66.4} & urd\_Latn & 11.3 & \textbf{12.9} & uzb\_Cyrl & \textbf{88.2} & 83.1 & uzb\_Latn & \textbf{70.7} & 66.9 \\
ven\_Latn & \textbf{76.0} & 68.0 & vie\_Latn & \textbf{90.0} & 88.7 & wal\_Ethi & 5.8 & \textbf{8.4} & wal\_Latn & \textbf{49.3} & 14.2 \\
wbm\_Latn & \textbf{71.6} & 18.0 & wol\_Latn & \textbf{32.4} & 28.4 & xav\_Latn & \textbf{7.6} & 6.0 & xho\_Latn & \textbf{58.9} & 48.7 \\
yao\_Latn & \textbf{46.4} & 17.1 & yap\_Latn & \textbf{22.2} & 11.6 & yom\_Latn & \textbf{46.9} & 30.0 & yor\_Latn & \textbf{58.7} & 12.4 \\
yue\_Hani & 13.1 & \textbf{79.8} & zai\_Latn & \textbf{27.8} & 27.1 & zho\_Hani & \textbf{47.8} & 47.8 & zlm\_Latn & \textbf{96.7} & 96.4 \\
zsm\_Latn & 91.8 & \textbf{96.2} & zul\_Latn & \textbf{90.9} & 66.7 \\

    \bottomrule
    \end{tabular}
}
    \caption{Top-10 accuracy of \frameworkname on \textbf{SR-B} using English and the closest donor language as source (Part II).}\label{tab:srb_donor_table2}
\end{table*}

==> tatoeba_donor.tex <==
\begin{table*}
\centering
\setlength{\tabcolsep}{0.7mm}{}
\resizebox{\textwidth}{!}{
    \begin{tabular}{lrr|lrr|lrr|lrr}
    \toprule
    Language & English & Closest donor &     Language & English & Closest donor &     Language & English & Closest donor &     Language & English & Closest donor \\
    \midrule
ace\_Arab & 2.5 & \textbf{3.0} & ace\_Latn & 48.0 & \textbf{52.7} & acm\_Arab & \textbf{93.8} & 87.1 & acq\_Arab & \textbf{94.0} & 94.0 \\
afr\_Latn & \textbf{95.8} & 84.8 & ajp\_Arab & \textbf{96.6} & 90.0 & aka\_Latn & \textbf{28.6} & 24.9 & als\_Latn & \textbf{91.4} & 91.4 \\
apc\_Arab & \textbf{94.3} & 88.4 & arb\_Arab & \textbf{94.8} & 94.8 & arb\_Latn & 4.2 & \textbf{5.0} & ars\_Arab & \textbf{94.6} & 94.6 \\
arz\_Arab & 91.0 & \textbf{99.2} & asm\_Beng & 71.2 & \textbf{73.8} & ast\_Latn & 95.5 & \textbf{99.4} & awa\_Deva & \textbf{78.2} & 78.2 \\
azb\_Arab & \textbf{46.7} & 34.3 & azj\_Latn & 96.4 & \textbf{98.1} & bak\_Cyrl & 82.7 & \textbf{91.7} & bam\_Latn & \textbf{25.4} & 24.4 \\
bel\_Cyrl & 70.1 & \textbf{91.5} & bem\_Latn & \textbf{36.4} & 30.8 & ben\_Beng & 85.4 & \textbf{93.9} & bho\_Deva & \textbf{73.5} & 73.5 \\
bjn\_Latn & 86.2 & \textbf{89.6} & bod\_Tibt & 33.0 & \textbf{36.6} & bos\_Latn & \textbf{99.3} & 98.9 & bug\_Latn & 15.9 & \textbf{16.0} \\
cat\_Latn & 94.5 & \textbf{99.5} & ceb\_Latn & \textbf{76.8} & 65.0 & ces\_Latn & \textbf{95.7} & 90.6 & cjk\_Latn & \textbf{16.8} & 13.1 \\
crh\_Latn & 76.5 & \textbf{88.2} & cym\_Latn & \textbf{67.5} & 55.2 & dan\_Latn & \textbf{99.3} & 96.2 & deu\_Latn & \textbf{98.3} & 98.3 \\
dyu\_Latn & \textbf{9.8} & 6.7 & dzo\_Tibt & 22.9 & \textbf{24.4} & ell\_Grek & \textbf{79.2} & 64.1 & eng\_Latn & \textbf{100.0} & 100.0 \\
est\_Latn & \textbf{95.1} & 93.1 & eus\_Latn & 82.8 & \textbf{88.6} & ewe\_Latn & \textbf{29.6} & 28.5 & fao\_Latn & \textbf{86.2} & 76.1 \\
fin\_Latn & \textbf{93.6} & 88.0 & fon\_Latn & \textbf{13.9} & 10.6 & fra\_Latn & \textbf{94.2} & 94.2 & fur\_Latn & 68.2 & \textbf{83.8} \\
gaz\_Latn & \textbf{28.2} & 28.2 & gla\_Latn & \textbf{25.7} & 25.7 & gle\_Latn & 45.9 & \textbf{61.1} & glg\_Latn & 98.5 & \textbf{99.8} \\
guj\_Gujr & 90.2 & \textbf{97.8} & hat\_Latn & \textbf{85.7} & 84.8 & hau\_Latn & \textbf{60.1} & 55.9 & heb\_Hebr & 95.8 & \textbf{97.2} \\
hne\_Deva & \textbf{81.8} & 80.7 & hrv\_Latn & 98.5 & \textbf{99.4} & hun\_Latn & \textbf{92.3} & 88.2 & hye\_Armn & 88.9 & \textbf{95.5} \\
ilo\_Latn & \textbf{59.2} & 50.4 & ind\_Latn & \textbf{99.7} & 99.7 & isl\_Latn & 85.9 & \textbf{91.2} & ita\_Latn & 97.0 & \textbf{99.2} \\
jpn\_Jpan & \textbf{94.7} & 94.7 & kab\_Latn & \textbf{9.7} & 9.6 & kac\_Latn & \textbf{19.9} & 17.8 & kam\_Latn & 19.3 & \textbf{24.8} \\
kas\_Arab & \textbf{9.0} & 9.0 & kas\_Deva & \textbf{7.6} & 7.6 & kat\_Geor & 84.7 & \textbf{86.7} & kaz\_Cyrl & 95.0 & \textbf{97.0} \\
kea\_Latn & \textbf{68.1} & 68.1 & khk\_Cyrl & 90.9 & \textbf{91.6} & khm\_Khmr & \textbf{65.4} & 65.4 & kik\_Latn & 26.0 & \textbf{37.5} \\
kir\_Cyrl & 90.9 & \textbf{94.8} & kmb\_Latn & \textbf{18.8} & 14.6 & kmr\_Latn & 58.5 & \textbf{60.1} & knc\_Arab & \textbf{2.6} & 2.6 \\
kon\_Latn & \textbf{44.7} & 37.8 & kor\_Hang & 95.3 & \textbf{98.2} & lao\_Laoo & \textbf{83.1} & 77.3 & lij\_Latn & \textbf{54.2} & 40.5 \\
lin\_Latn & 54.0 & \textbf{66.0} & lit\_Latn & 90.0 & \textbf{94.4} & lmo\_Latn & 39.3 & \textbf{51.8} & ltg\_Latn & \textbf{18.9} & 18.9 \\
lua\_Latn & \textbf{31.7} & 31.3 & lug\_Latn & \textbf{33.1} & 22.2 & luo\_Latn & 22.6 & \textbf{26.8} & lus\_Latn & \textbf{39.2} & 39.2 \\
mag\_Deva & \textbf{78.1} & 63.0 & mai\_Deva & \textbf{87.2} & 76.2 & mal\_Mlym & 80.8 & \textbf{84.0} & mar\_Deva & 91.9 & \textbf{97.8} \\
min\_Latn & 71.6 & \textbf{76.2} & mkd\_Cyrl & 96.8 & \textbf{99.3} & mlt\_Latn & \textbf{70.3} & 70.3 & mni\_Beng & \textbf{2.2} & 2.2 \\
mri\_Latn & \textbf{35.6} & 28.9 & mya\_Mymr & \textbf{41.2} & 38.8 & nld\_Latn & \textbf{97.0} & 90.2 & nno\_Latn & \textbf{98.6} & 98.6 \\
npi\_Deva & 95.9 & \textbf{98.0} & nso\_Latn & \textbf{45.2} & 45.2 & nus\_Latn & \textbf{3.3} & 2.8 & nya\_Latn & \textbf{55.4} & 37.0 \\
ory\_Orya & \textbf{77.2} & 73.8 & pag\_Latn & \textbf{70.6} & 60.7 & pan\_Guru & \textbf{53.1} & 53.1 & pap\_Latn & \textbf{85.9} & 84.6 \\
pes\_Arab & \textbf{98.6} & 98.2 & plt\_Latn & 41.5 & \textbf{59.2} & pol\_Latn & 92.7 & \textbf{97.7} & por\_Latn & 99.0 & \textbf{99.8} \\
quy\_Latn & 40.5 & \textbf{41.3} & ron\_Latn & 94.8 & \textbf{99.2} & run\_Latn & 44.1 & \textbf{61.0} & rus\_Cyrl & \textbf{98.0} & 98.0 \\
san\_Deva & 46.2 & \textbf{69.6} & sat\_Olck & 22.6 & \textbf{23.9} & scn\_Latn & \textbf{65.4} & 50.7 & shn\_Mymr & 1.6 & \textbf{1.9} \\
slk\_Latn & \textbf{94.1} & 88.0 & slv\_Latn & 95.4 & \textbf{97.2} & smo\_Latn & \textbf{31.4} & 19.7 & sna\_Latn & 40.2 & \textbf{40.4} \\
som\_Latn & 38.8 & \textbf{43.0} & sot\_Latn & \textbf{45.3} & 36.1 & spa\_Latn & \textbf{95.4} & 95.4 & srd\_Latn & \textbf{64.9} & 51.3 \\
ssw\_Latn & \textbf{43.4} & 38.5 & sun\_Latn & 89.8 & \textbf{93.4} & swe\_Latn & \textbf{99.9} & 96.4 & swh\_Latn & \textbf{91.0} & 91.0 \\
tam\_Taml & \textbf{79.4} & 79.4 & taq\_Latn & \textbf{8.6} & 7.6 & taq\_Tfng & \textbf{1.1} & 1.0 & tat\_Cyrl & 93.0 & \textbf{97.2} \\
tgk\_Cyrl & \textbf{75.0} & 75.0 & tgl\_Latn & \textbf{86.4} & 77.3 & tha\_Thai & 94.5 & \textbf{96.3} & tir\_Ethi & \textbf{23.4} & 23.4 \\
tsn\_Latn & 31.3 & \textbf{35.8} & tso\_Latn & \textbf{38.0} & 32.4 & tuk\_Latn & 68.2 & \textbf{80.8} & tum\_Latn & \textbf{34.5} & 26.5 \\
twi\_Latn & \textbf{41.6} & 35.8 & tzm\_Tfng & \textbf{0.9} & 0.9 & uig\_Arab & 70.1 & \textbf{80.2} & ukr\_Cyrl & 96.6 & \textbf{99.3} \\
urd\_Arab & 93.0 & \textbf{96.9} & uzn\_Latn & 83.2 & \textbf{88.6} & vec\_Latn & 81.7 & \textbf{89.3} & vie\_Latn & \textbf{97.5} & 92.3 \\
wol\_Latn & 18.6 & \textbf{18.8} & xho\_Latn & 48.7 & \textbf{52.1} & ydd\_Hebr & \textbf{51.0} & 32.8 & yor\_Latn & \textbf{25.3} & 16.2 \\
zho\_Hans & 98.4 & \textbf{99.6} & zho\_Hant & \textbf{98.7} & 98.7 & zsm\_Latn & \textbf{99.5} & 100.0 & zul\_Latn & \textbf{60.7} & 58.7 \\

    \bottomrule
    \end{tabular}
}
    \caption{Top-10 accuracy of \frameworkname on \textbf{FLORES-200} using English and the closest donor languages as source.}\label{tab:flores_donor_table1}
\end{table*}
